BFS-Net: Weakly Supervised Cell Instance Segmentation from Bright-Field Microscopy Z-Stacks

Despite its broad availability, volumetric information acquisition from Bright-Field Microscopy (BFM) is inherently difficult due to the projective nature of the acquisition process. We investigate the prediction of 3D cell instances from a set of BFM Z-Stack images. We propose a novel two-stage weakly supervised method for volumetric instance segmentation of cells which only requires approximate cell centroids annotation. Created pseudo-labels are thereby refined with a novel refinement loss with Z-stack guidance. The evaluations show that our approach can generalize not only to BFM Z-Stack data, but to other 3D cell imaging modalities. A comparison of our pipeline against fully supervised methods indicates that the significant gain in reduced data collection and labelling results in minor performance difference.

==> 3-0-dataset.tex <==
In absence of a publicly available dataset for this specific use case, we collected a BFM Z-Stack dataset of SF-9 insect cells (ThermoFisher, Germany), and roughly annotated the geometric centers of the cells. In order to decrease the sedimentation speed of the cells, cells were suspended in feeding medium supplemented with 20\% Fetal Calf Serum (FCS). BFM images were obtained using Zeiss Axiovert 40 CFL microscope with 20x magnification.
The dataset consists of 120 instances of $64\times256\times256$ with z-spacing of 2 $\mu m$ per slice. We crop the instances to 16 slices for training and resize each plane to a $128\times128$ image. The data is splitted to a 4:1 train/validation split. The dataset will be made publicly available upon acceptance.


